Multi-Task Learning with Group-Specific Feature Space Sharing

When faced with learning a set of inter-related tasks from a limited amount of usable data, learning each task independently may lead to poor generalization performance. Multi-Task Learning (MTL) exploits the latent relations between tasks and overcomes data scarcity limitations by co-learning all these tasks simultaneously to offer improved performance. We propose a novel Multi-Task Multiple Kernel Learning framework based on Support Vector Machines for binary classification tasks. By considering pair-wise task affinity in terms of similarity between a pair's respective feature spaces, the new framework, compared to other similar MTL approaches, offers a high degree of flexibility in determining how similar feature spaces should be, as well as which pairs of tasks should share a common feature space in order to benefit overall performance. The associated optimization problem is solved via a block coordinate descent, which employs a consensus-form Alternating Direction Method of Multipliers algorithm to optimize the Multiple Kernel Learning weights and, hence, to determine task affinities. Empirical evaluation on seven data sets exhibits a statistically significant improvement of our framework's results compared to the ones of several other Clustered Multi-Task Learning methods.

==> TitleAuthors.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\MYTITLE}{Multi-Task Learning with Group-Specific\texorpdfstring{\\}{} Feature Space Sharing}

% The \ecmltitle you define below is probably too long as a header.
% Therefore, a short form for the running title is supplied here:
%\title{Multi-Task Learning with Unrestricted Task Affinity}
\title{\MYTITLE}

\author{Niloofar Yousefi\inst{1} \and Michael Georgiopoulos\inst{1} \and \\ Georgios C. Anagnostopoulos\inst{2}}

\institute{University of Central Florida, Department of Electrical Engineering \& Computer Science, 4000 Central Florida Blvd, Orlando, Florida, 32816, USA \\
\email{niloofar.yousefi@ucf.edu, michaelg@ucf.edu}
\and Florida Institute of Technology, Department of Electrical and Computer Engineering,\\ 150 W. University Blvd, Melbourne, FL 32901, USA \\
\email{georgio@fit.edu}}


